Evidence for environmental effects in the $z\,{=}\,4.3$ protocluster core SPT2349$-$56

We present ALMA observations of the [CI] 492 and 806$\,$GHz fine-structure lines in 25 dusty star-forming galaxies (DSFGs) at $z\,{=}\,4.3$ in the core of the SPT2349$-$56 protocluster. The protocluster galaxies exhibit a median $L^\prime_{[\text{CI}](2-1)}/L^\prime_{[\text{CI}](1-0)}$ ratio of 0.94 with an interquartile range of 0.81-1.24. These ratios are markedly different to those observed in DSFGs in the field (across a comparable redshift and 850$\,\mu$m flux density range), where the median is 0.55 with an interquartile range of 0.50-0.76, and we show that this difference is driven by an excess of [CI](2-1) in the protocluster galaxies for a given 850$\,\mu$m flux density. Assuming local thermal equilibrium, we estimate gas excitation temperatures of $T_{\rm ex}\,{=}\,59.1^{+8.1}_{-6.8}\,$K for our protocluster sample and $T_{\rm ex}\,{=}\,33.9^{+2.4}_{-2.2}\,$K for the field sample. Our main interpretation of this result is that the protocluster galaxies have had their cold gas driven to their cores via close-by interactions within the dense environment, leading to an overall increase in the average gas density and excitation temperature, and an elevated [CI](2-1) luminosity-to-far-infrared luminosity ratio.

==> Tables/line_table.tex <==
%\begin{table}
%\centering
%\caption{Summary of the line measurements and Band 4 aperture radii ($R$). The uncertainties are $1\sigma$. Measurements below $2\sigma$ are shown as $3\sigma$ upper bounds.}
%\label{tab:lines}
%\begin{tabular}{c c c c}
%\toprule
% ID & $L_{\rm [CI](1-0)}$ & $L_{\rm [CI](2-1)}$ & $L_{\rm CO(7-6)}$ \\
%    & ($\mathrm{10^7 L_\odot}$) & ($\mathrm{10^7 L_\odot}$) & ($\mathrm{10^7 L_\odot}$) \\
%\hline
%\multicolumn{4}{c}{Core}\\
%\hline
%C1 & 3.86 $\pm$ 0.41 & 27.7 $\pm$ 2.4 & 34.7 $\pm$ 2.3 \\
%C2 & 0.63 $\pm$ 0.28 & 3.4 $\pm$ 1.2 & 7.8 $\pm$ 1.0 \\
%C3 & 4.01 $\pm$ 0.33 & 17.7 $\pm$ 1.1 & 23.7 $\pm$ 1.0 \\
%C4 & 3.01 $\pm$ 0.39 & 12.0 $\pm$ 1.8 & 8.9 $\pm$ 1.7 \\
%C5 & 2.56 $\pm$ 0.39 & 9.0 $\pm$ 1.9 & 7.0 $\pm$ 1.7 \\
%C6 & 2.12 $\pm$ 0.25 & 11.56 $\pm$ 0.63 & 19.49 $\pm$ 0.67 \\
%C7 & 1.18 $\pm$ 0.23 & 4.00 $\pm$ 0.89 & 5.67 $\pm$ 0.86 \\
%C8 & 1.03 $\pm$ 0.30 & 9.8 $\pm$ 1.3 & 12.0 $\pm$ 1.3 \\
%C9 & 1.31 $\pm$ 0.31 & 3.64 $\pm$ 0.89 & 9.42 $\pm$ 0.87 \\
%C10 & 0.68 $\pm$ 0.32 & 7.55 $\pm$ 0.89 & 10.90 $\pm$ 0.87 \\
%C11 & $<$0.8 & $<$3.14 & 3.76 $\pm$ 0.71 \\
%C12 & $<$0.88 & $<$0.42 & $<$0.51% 0.224 $\pm$ 0.096
% \\
%C13 & 0.42 $\pm$ 0.15 & 3.91 $\pm$ 0.91 & 6.06 $\pm$ 0.90 \\
%C14 & $<$0.88 & $<$1.7 & $<$2.86 \\
%C15 & 1.10 $\pm$ 0.26 & 6.1 $\pm$ 1.7 & 4.4 $\pm$ 1.5 \\
%C16 & 0.62 $\pm$ 0.21 & $<$1.25 & $<$1.14 \\
%C17 & $<$0.56 & $<$1.62 & $<$1.42 \\
%C18 & $<$0.85 & $<$3.55 & $<$2.09 \\
%C19 & 0.79 $\pm$ 0.28 & $<$4.52 & $<$5.0 \\
%C20 & $<$0.73 & $<$1.36 & $<$1.5 \\
%C21 & 0.43 $\pm$ 0.14 & $<$1.15 & $<$1.14 \\
%C22 & 0.138 $\pm$ 0.065 & $<$0.81 & $<$1.05 \\
%C23 & $<$0.71 & $<$1.04 & $<$1.04 \\
%C24 & 0.72 $\pm$ 0.21 & $<$2.96 & 3.09 $\pm$ 0.92 \\
%C25 & $<$0.85 & $<$1.96 & 1.44 $\pm$ 0.53 \\
%C26 & $<$1.0 & 1.55 $\pm$ 0.76 & $<$2.12 \\
%C27 & $<$0.21 & $<$0.64 & 0.43 $\pm$ 0.16 \\
%C28 & $<$0.43 & $<$0.55 & $<$0.72 \\
%C29 & 0.32 $\pm$ 0.11 & $<$0.45 & $<$0.41 \\
%C30 & $<$0.45 & $<$1.14 & $<$0.85 \\
%C31 & $<$0.96 & $<$2.16 & 1.84 $\pm$ 0.66 \\
%\hline
%\multicolumn{4}{c}{North} \\
%\hline
% N1 & 6.68 $\pm$ 0.37 & 25.5 $\pm$ 3.6 & 59.8 $\pm$ 3.6 \\
%N2 & 2.72 $\pm$ 0.45 & 23.0 $\pm$ 6.4 & 13.8 $\pm$ 6.4 \\
%\hline
%\end{tabular}
%\end{table}


\begin{table}
\centering
\caption{Summary of the observed line strength measurements. The uncertainties are $1\sigma$. Measurements below $2\sigma$ are shown as $3\sigma$ upper bounds. The line luminosities shown in Fig.~\ref{fig:linestrength} are derived from line strengths using $L\,{=}\,4 \pi D_{\rm L}(z)^2F$, with $D_{\rm L}(z)$ being the the luminosity distance at $z\,{=}\,4.303$ and $F$ being the line strength in SI units. Line strengths in SI units are calculated using the values in this table as $F\,[\mathrm{W\,m^{-2}}]\,{=}\,F\,[\mathrm{Jy\,km\,s^{-1}}]\frac{\nu_{\rm em}}{c(1\,{+}\,z)} 10^{-26}$, where $\nu_{\rm em}$ is the emitted frequency of the line and $c$ is the speed of light.}
\label{tab:lines}
\begin{tabular}{c c c c}
\toprule
 ID & $F_{\rm [CI](1-0)}$ & $F_{\rm [CI](2-1)}$ & $F_{\rm CO(7-6)}$ \\
    & (Jy\,km\,s$^{-1}$) & (Jy\,km\,s$^{-1}$) & (Jy\,km\,s$^{-1}$) \\
\hline
\multicolumn{4}{c}{Core}\\
\hline
C1 & 0.250 $\pm$ 0.026 & 1.089 $\pm$ 0.094 & 1.371 $\pm$ 0.089 \\
C2 & 0.041 $\pm$ 0.018 & 0.132 $\pm$ 0.047 & 0.307 $\pm$ 0.041 \\
C3 & 0.259 $\pm$ 0.021 & 0.698 $\pm$ 0.045 & 0.937 $\pm$ 0.040 \\
C4 & 0.195 $\pm$ 0.025 & 0.471 $\pm$ 0.071 & 0.351 $\pm$ 0.066 \\
C5 & 0.165 $\pm$ 0.025 & 0.355 $\pm$ 0.073 & 0.276 $\pm$ 0.067 \\
C6 & 0.137 $\pm$ 0.016 & 0.455 $\pm$ 0.025 & 0.769 $\pm$ 0.026 \\
C7 & 0.076 $\pm$ 0.015 & 0.157 $\pm$ 0.035 & 0.224 $\pm$ 0.034 \\
C8 & 0.067 $\pm$ 0.020 & 0.387 $\pm$ 0.053 & 0.472 $\pm$ 0.051 \\
C9 & 0.085 $\pm$ 0.020 & 0.143 $\pm$ 0.035 & 0.372 $\pm$ 0.034 \\
C10 & 0.044 $\pm$ 0.021 & 0.297 $\pm$ 0.035 & 0.430 $\pm$ 0.034 \\
C11 & $<$0.052 & $<$0.123 & 0.148 $\pm$ 0.028 \\
C12 & $<$0.057 & $<$0.016 & $<$0.020 \\
C13 & 0.027 $\pm$ 0.010 & 0.154 $\pm$ 0.036 & 0.239 $\pm$ 0.036 \\
C14 & $<$0.057 & $<$0.067 & $<$0.113 \\
C15 & 0.071 $\pm$ 0.017 & 0.239 $\pm$ 0.068 & 0.173 $\pm$ 0.059 \\
C16 & 0.040 $\pm$ 0.014 & $<$0.049 & $<$0.045 \\
C17 & $<$0.036 & $<$0.064 & $<$0.056 \\
C18 & $<$0.055 & $<$0.140 & $<$0.083 \\
C19 & 0.051 $\pm$ 0.018 & $<$0.178 & $<$0.197 \\
C20 & $<$0.048 & $<$0.053 & $<$0.059 \\
C21 & 0.028 $\pm$ 0.009 & $<$0.045 & $<$0.045 \\
C22 & 0.009 $\pm$ 0.004 & $<$0.032 & $<$0.042 \\
C23 & $<$0.046 & $<$0.041 & $<$0.041 \\
%C24 & 0.046 $\pm$ 0.014 & $<$0.117 & 0.122 $\pm$ 0.036 \\
%C25 & $<$0.055 & $<$0.077 & 0.057 $\pm$ 0.021 \\
%C26 & $<$0.064 & 0.061 $\pm$ 0.030 & $<$0.084 \\
%C27 & $<$0.014 & $<$0.025 & 0.017 $\pm$ 0.006 \\
%C28 & $<$0.028 & $<$0.021 & $<$0.028 \\
%C29 & 0.021 $\pm$ 0.007 & $<$0.018 & $<$0.016 \\
%C30 & $<$0.029 & $<$0.045 & $<$0.033 \\
%C31 & $<$0.062 & $<$0.085 & 0.073 $\pm$ 0.026 \\
\hline
\multicolumn{4}{c}{North} \\
\hline
% N1 & 0.431 $\pm$ 0.024 & 1.000 $\pm$ 0.141 & 2.353 $\pm$ 0.142 \\
% N2 & 0.175 $\pm$ 0.029 & 0.902 $\pm$ 0.251 & 0.543 $\pm$ 0.252 \\
N1 & 0.432 $\pm$ 0.024 & 0.998 $\pm$ 0.101 & 2.356 $\pm$ 0.101 \\
N2 & 0.202 $\pm$ 0.029 & 0.905 $\pm$ 0.183 & 0.547 $\pm$ 0.182 \\
\hline
\end{tabular}
\end{table}

==> Tables/line_table_old.tex <==
\begin{table}
\centering
\caption{Summary of the line measurements and band 4 aperture radii ($R$). The uncertainties are $1\sigma$, and the upper bounds are $3\sigma$.}
\begin{tabular}{c c c c c}
\toprule
 ID & $L_{\rm CI(1-0)}$ & $L_{\rm CI(2-1)}$ & $L_{\rm CO(7-6)}$ & $R$ \\
    & ($\mathrm{10^7 L_\odot}$) & ($\mathrm{10^7 L_\odot}$) & ($\mathrm{10^7 L_\odot}$) & (arcsec.)\\
\hline
\multicolumn{5}{c}{Core}\\
\hline
C1 & 3.79 $\pm$ 0.42 & 27.6 $\pm$ 3.3 & 34.8 $\pm$ 3.1 & 1.12 \\
C2 & $<$0.91 & $<$8.92 & 9.0 $\pm$ 1.9 & 1 \\
C3 & 2.86 $\pm$ 0.33 & 16.6 $\pm$ 1.6 & 22.3 $\pm$ 1.4 & 0.65 \\
C4 & 2.50 $\pm$ 0.40 & 11.9 $\pm$ 2.6 & 8.8 $\pm$ 2.4 & 0.8 \\
C5 & 1.90 $\pm$ 0.41 & 7.8 $\pm$ 2.4 & 6.1 $\pm$ 2.3 & 0.85 \\
C6 & 2.12 $\pm$ 0.27 & 11.6 $\pm$ 1.0 & 19.5 $\pm$ 1.0 & 0.6 \\
C7 & 0.60 $\pm$ 0.25 & 4.2 $\pm$ 1.5 & 5.9 $\pm$ 1.4 & 0.85 \\
C8 & 0.91 $\pm$ 0.32 & 9.9 $\pm$ 1.9 & 12.0 $\pm$ 1.8 & 0.7 \\
C9 & 0.67 $\pm$ 0.33 & 3.5 $\pm$ 1.5 & 9.5 $\pm$ 1.5 & 0.65 \\
C10 & 0.70 $\pm$ 0.34 & 9.7 $\pm$ 2.2 & 8.2 $\pm$ 2.1 & 1 \\
C11 & $<$0.87 & $<$4.46 & 3.8 $\pm$ 1.1 & 0.6 \\
C12 & $<$0.72 & $<$0.77 & $<$0.83 & 0.15 \\
C13 & 0.71 $\pm$ 0.35 & 3.9 $\pm$ 1.4 & 6.1 $\pm$ 1.4 & 0.55 \\
C14 & $<$0.88 & $<$4.5 & $<$5.6 & 1 \\
C15 & $<$0.87 & 6.1 $\pm$ 2.5 & 4.4 $\pm$ 2.2 & 0.9 \\
C16 & 0.52 $\pm$ 0.24 & $<$1.82 & $<$1.75 & 0.3 \\
C17 & $<$0.59 & $<$2.44 & $<$2.32 & 0.5 \\
C18 & $<$0.8 & $<$4.6 & $<$2.83 & 0.4 \\
C19 & $<$1.56 & $<$11.76 & $<$15.58 & 1 \\
C20 & $<$0.62 & $<$1.96 & $<$1.83 & 0.4 \\
C21 & $<$0.55 & $<$3.57 & $<$3.56 & 1 \\
C22 & $<$0.39 & $<$1.25 & $<$1.59 & 0.4 \\
C23 & $<$0.58 & $<$2.09 & $<$1.97 & 0.6 \\
C24 & 0.66 $\pm$ 0.26 & $<$8.07 & $<$9.36 & 1 \\
C25 & $<$0.71 & $<$2.37 & $<$3.55 & 0.4 \\
C26 & $<$0.79 & $<$6.78 & $<$4.1 & 0.7 \\
C27 & $<$0.4 & $<$1.2 & $<$1.45 & 0.35 \\
C28 & $<$0.55 & $<$1.05 & $<$1.23 & 0.3 \\
C29 & $<$0.74 & $<$0.9 & $<$0.82 & 0.25 \\
C30 & $<$0.46 & $<$1.88 & $<$1.59 & 0.6 \\
C31 & $<$1.08 & $<$3.33 & $<$5.01 & 0.5 \\
\hline
\multicolumn{5}{c}{North} \\
\hline
N1 & 6.68 $\pm$ 0.38 & 25.5 $\pm$ 3.6 & 59.8 $\pm$ 3.6 & 1.1 \\
N2 & 2.72 $\pm$ 0.46 & 23.0 $\pm$ 6.4 & 13.8 $\pm$ 6.4 & 1.1 \\
\hline
\end{tabular}
\end{table}

==> Tables/newlocs_2sigma_table.tex <==
\begin{tabular}{c c c c c}
\toprule
 & $\mathrm{L_{[CI](1-0)}}$ & $\mathrm{L_{[CI](2-1)}}$ & $\mathrm{L_{CO(7-6)}}$ & R \\
\midrule
C1 & 3.86 $\pm$ 0.41 & 27.7 $\pm$ 2.4 & 34.7 $\pm$ 2.3 & 1.12 \\
C2 & 0.63 $\pm$ 0.28 & 3.4 $\pm$ 1.2 & 7.8 $\pm$ 1.0 & 0.8 \\
C3 & 4.01 $\pm$ 0.33 & 17.7 $\pm$ 1.1 & 23.7 $\pm$ 1.0 & 0.65 \\
C4 & 3.01 $\pm$ 0.39 & 12.0 $\pm$ 1.8 & 8.9 $\pm$ 1.7 & 0.8 \\
C5 & 2.56 $\pm$ 0.39 & 9.0 $\pm$ 1.9 & 7.0 $\pm$ 1.7 & 0.9 \\
C6 & 2.12 $\pm$ 0.25 & 11.56 $\pm$ 0.63 & 19.49 $\pm$ 0.67 & 0.6 \\
C7 & 1.18 $\pm$ 0.23 & 4.00 $\pm$ 0.89 & 5.67 $\pm$ 0.86 & 0.8 \\
C8 & 1.03 $\pm$ 0.30 & 9.8 $\pm$ 1.3 & 12.0 $\pm$ 1.3 & 0.7 \\
C9 & 1.31 $\pm$ 0.31 & 3.64 $\pm$ 0.89 & 9.42 $\pm$ 0.87 & 0.6 \\
C10 & 0.68 $\pm$ 0.32 & 7.55 $\pm$ 0.89 & 10.90 $\pm$ 0.87 & 0.6 \\
C11 & $<$0.8 & $<$3.14 & 3.76 $\pm$ 0.71 & 0.6 \\
C12 & $<$0.88 & $<$0.42 & 0.224 $\pm$ 0.096 & 0.15 \\
C13 & 1.73 $\pm$ 0.33 & 3.91 $\pm$ 0.91 & 6.06 $\pm$ 0.90 & 0.55 \\
C14 & $<$0.88 & $<$1.7 & $<$2.86 & 0.6 \\
C15 & 1.10 $\pm$ 0.26 & 6.1 $\pm$ 1.7 & 4.4 $\pm$ 1.5 & 0.9 \\
C16 & 0.62 $\pm$ 0.21 & $<$1.25 & $<$1.14 & 0.3 \\
C17 & $<$0.56 & $<$1.62 & $<$1.42 & 0.5 \\
C18 & $<$0.85 & $<$3.55 & $<$2.09 & 0.5 \\
C19 & 0.79 $\pm$ 0.28 & $<$4.52 & $<$5.0 & 0.6 \\
C20 & $<$0.73 & $<$1.36 & $<$1.5 & 0.5 \\
C21 & 0.43 $\pm$ 0.14 & $<$1.15 & $<$1.14 & 0.5 \\
C22 & 0.138 $\pm$ 0.065 & $<$0.81 & $<$1.05 & 0.5 \\
C23 & $<$0.71 & $<$1.04 & $<$1.04 & 0.5 \\
C24 & 0.72 $\pm$ 0.21 & $<$2.96 & 3.09 $\pm$ 0.92 & 0.55 \\
C25 & $<$0.85 & $<$1.96 & 1.44 $\pm$ 0.53 & 0.5 \\
C26 & $<$1.0 & 1.55 $\pm$ 0.76 & $<$2.12 & 0.6 \\
C27 & $<$0.21 & $<$0.64 & 0.43 $\pm$ 0.16 & 0.35 \\
C28 & $<$0.43 & $<$0.55 & $<$0.72 & 0.3 \\
C29 & 0.32 $\pm$ 0.11 & $<$0.45 & $<$0.41 & 0.25 \\
C30 & $<$0.45 & $<$1.14 & $<$0.85 & 0.6 \\
C31 & $<$0.96 & $<$2.16 & 1.84 $\pm$ 0.66 & 0.5 \\
N1 & 6.68 $\pm$ 0.37 & 25.4 $\pm$ 2.6 & 59.7 $\pm$ 2.6 & 1.1 \\
N2 & 3.12 $\pm$ 0.45 & 23.0 $\pm$ 4.6 & 13.9 $\pm$ 4.6 & 1.1 \\
\bottomrule
\end{tabular}

